An improved Branch-and-cut code for the maximum balanced subgraph of a signed graph

The Maximum Balanced Subgraph Problem (MBSP) is the problem of finding a subgraph of a signed graph that is balanced and maximizes the cardinality of its vertex set. We are interested in the exact solution of the problem: an improved version of a branch-and-cut algorithm is proposed. Extensive computational experiments are carried out on a set of instances from three applications previously discussed in the literature as well as on a set of random instances.

==> exact.tex <==

\section{Exact solution approach}
\label{sec:ExactSolution}

A branch-and-cut algorithm was recently proposed for the MBSP~\cite{Figueiredo11}.
In this section, we describe an improved version of this algorithm in which a new branching rule
and new separation routines are used.

\subsection{Integer programming formulation}

The integer programming formulation introduced in~\cite{Figueiredo11} is described next.
A signed graph is balanced if and only if it does not contain a parallel edge or
a cycle with an odd number of negative edges~\cite{barahona89}.
Let $C^o(E)$ be the set of all odd negative cycles in $G$, i.e., cycles with no parallel edges and with an odd
number of negative edges.
From now on, a cycle $C\in C^o(E)$ is called an {\it odd negative cycle}.
The formulation uses binary decision variables $y\in\{0,1\}^{|V|}$ defined in the following way.
For all $i\in V$, $y_i$ is equal to 1 if vertex $i\in V$ belongs to the balanced subgraph, and is
equal to 0 otherwise.

We use the vector notation $y=(y_i)$, $i\in V$, and the
notation $y(V')=\sum_{i\in V'} y_i$ for $V'\subseteq V$.
The formulation follows.
\begin{align}
\mathrm{Maximize\ }    & y(V)                      & \label{fo}\\
\mathrm{subject\ to\ } & y_i + y_j \leq 1, &\forall\ (i,j)\in E^-\cap E^+,
\label{paralEdge}\\
                       & y(C) \leq |C|-1,  &\forall\ C\in C^o(E), \label{C-oddIneq}\\
                       & y_i\in\{0,1\},    &\forall\ i\in V.\label{yInt}
\end{align}
Consider a parallel edge $(i,j)\in E^-\cap E^+$. Constraints~(\ref{paralEdge})
ensure vertices $i$ and $j$ cannot belong together to the balanced subgraph.
Constraints~(\ref{C-oddIneq}), called {\it odd negative cycle inequalities}, forbid cycles with an odd number of negative
edges in the subgraph described by variables $y$. These constraints
force variables $y$ to define a balanced subgraph while
the objective function (\ref{fo}) looks for a maximum balanced subgraph.
The formulation has $n$ variables and, due to constraints~(\ref{C-oddIneq}), might have an exponential
number of constraints.

\subsection{An improved branch-and-cut code}

The branch-and-cut algorithm developed in~\cite{Figueiredo11} has three basic
components: the initial formulation, the cut generation and the primal heuristic.
For a detailed description we refer the reader to the original work.
The following new routines were added to this branch-and-cut code.

\paragraph{\bf Branching on the odd negative cycle inequalities}
A standard 0–-1 branching rule was implemented in~\cite{Figueiredo11}. The authors reported that
a version of the branching rule proposed in~\cite{Balas86} was also implemented but, although it has been successfully
applied to the stable set problem~\cite{rebennack09,rossi01}, better results were obtained to the MBSP
with the standard 0-–1 branching rule.
Our branching rule is based on the odd negative cycle inequalities~(\ref{C-oddIneq}) and has shown to be
more efficient than the standard one.
Let $\bar{y}\in\mathbb{R}$ be the optimal fractional solution of a node in the search tree.
Let $C'\subseteq C^o(E)$ be the subset of odd negative cycles such that each cycle $C\in C'$ satisfy the following conditions:
constraint~(\ref{C-oddIneq}) defined by $C'$ is a binding one in the current formulation;
there exists a vertex $i\in \bar{C}$ such that $\bar{y}_i$ is fractional.
The standard 0--1 branching rule is used whenever $C'$ is an empty set.
If it is not the case, let $\bar{C}$ be the smallest cycle in $C'$.
Split $\bar{C}$ into the sets $\bar{C}^1$ and $\bar{C}^2$
such that $\bar{C} = \bar{C}^1\cup \bar{C}^2$, $\bar{C}^1\cap \bar{C}^2=\emptyset$ and $y(\bar{C}^1)$ is fractional.
We create three branches in the search tree:
(i)  $y(\bar{C}^1) \leq  |\bar{C}^1|-1$ and $y(\bar{C}^2) = |\bar{C}^2|$;
(ii)  $y(\bar{C}^1) =  |\bar{C}^1|$ and $y(\bar{C}^2)\leq |\bar{C}^2|-1$;
(iii) $y(\bar{C}^1) \leq  |\bar{C}^1|-1$ and $y(\bar{C}^2)\leq |\bar{C}^2|-1$.

\paragraph{\bf Separation routines}
The cut generation component described in~\cite{Figueiredo11} has two separation procedures: an
exact separation procedure for odd negative cycle inequalities~(\ref{C-oddIneq}) and
a heuristic separation procedure for a family of clique inequalities introduced in~\cite{Figueiredo11}.
In this work, we have implemented these two separation procedures.
We have also added two new procedures to the cut generation component.
We have implemented the separation procedure described in~\cite{padberg73} to the lifted odd hole inequalities
defined over the set of parallel edges.
Moreover, as indicated in~\cite{Figueiredo11}, in order to strengthen constraints~(\ref{C-oddIneq}),
we have implemented a lifting procedure to the odd negative cycle inequalities with
$|C|\leq 20$. In both cases, the subproblems appearing in each iteration of the lifting procedure
were solved by simple enumerative algorithms.


==> heuri.tex <==

\section{Heuristic solution approaches}
\label{sec:HeuristicSolution}

In this section, we describe two heuristic approaches to the MBSP: a greedy heuristic proposed in~\cite{gulpinarI} for the DMERN problem and a GRASP metaheuristic introduced in this work.

\subsection{GGMZ greedy heuristic}

The heuristic proposed by Gulpinar {\it et al.}~\cite{gulpinarI} is described in Algorithm~\ref{alg:gulp} and is motivated by the following basic result.
\begin{lmm}{\cite{gulpinarI}}
Every signed tree $T=(V_T,E_T)$ is a balanced graph.
\label{teo:gulp}
\end{lmm}
%\begin{proof}
%The theorem is proven by induction on the number of edges in $T$. The theorem is clearly true when $\mid E_T \mid = 1$. Let $i \in V_T$
%be a vertex of degree $1$ in $T$. By induction, there is a set $W \subset V_T \backslash \{i\}$ such that $(T-\{i\})^W$ has no negative edges.
%In $T^W$, the edge incident to $i$ is positive or negative. In the first case, let $W' = W$ and the second case, let $W'=W \cup \{i\}$. Then, $T^{W'}$ has no negative edges.
%\end{proof}

%Theorem \ref{teo:gulp} motivates the heuristic depicted in Algorithm~\ref{alg:gulp}.

\begin{algorithm}[tbh]
\small
%\SetLine
  \KwIn{signed graph $G=(V,E,s)$}
  \KwOut{stable set $I$}

  Find a spanning tree $T$ in $G$\;
  Compute a subset $W \subseteq V$ such that $T^W$ has no negative edges\;
  Find a maximal stable set $I$ in the graph $(G^W)^-$\;

  return $I$\;
\caption{{\sc GGMZ greedy heuristic.}}
\label{alg:gulp}
\end{algorithm}

It is not difficult to see that there always exists a partition of set $I$ into two subsets that represents a feasible solution for the MBSP.
%Notice that, if the stable set $I=V$, then $G$ is a balanced graph.
The greedy heuristic proposed by Gulpinar {\it et al.} has the advantage to find the optimal solution of the MBSP whenever $G$ is a balanced graph.

The first step of Algorithm~\ref{alg:gulp} could be implemented in a number of different ways.
In \cite{gutin09}, the authors tried three well known strategies to construct a spanning tree:
Breadth First Search ($BFS$), Depth First Search ($DFS$) and a random method.
Following similar ideas, the Step 1 is implemented in this work as a $BFS$, a $DFS$ and by using other five different spanning tree strategies.
In these additional strategies, we calculate a minimum spanning tree based on costs generated for each edge $e$
of the graph. The Kruskal algorithm~\cite{cormen09} is used to calculate the minimum spanning tree and the
following cost functions were designed:

\begin{itemize}
\item $(-,+-,+)$: $f_1(e) = \{ 3$ if $e \in E^+\setminus E^-$; $1$ if $e \in E^-\setminus E^+$; $2$ if $e \in (E^- \cap E^+) \}$;
\vspace{-.2cm}
\item $(+,-,+-)$: $f_2(e) = \{ 1$ if $e \in E^+\setminus E^-$; $2$ if $e \in E^-\setminus E^+$; $3$ if $e \in (E^- \cap E^+) \}$;
\vspace{-.2cm}
\item $(-,+,+-)$: $f_3(e) = \{ 2$ if $e \in E^+\setminus E^-$; $1$ if $e \in E^-\setminus E^+$; $3$ if $e \in (E^- \cap E^+) \}$;
\vspace{-.2cm}
\item Random: a random function $f_{random}(e) \in [0, 1000]$;
\vspace{-.2cm}
\item Adaptive: an adaptive function $f_{Adapt}(e) = \{ f_1(e)$ if $|E^-|/|E^+| < 1$; $f_2(e)$ otherwise$\}$.
\end{itemize}

In Step $2$, the subset $W$ is found by using a recursive procedure based on the inductive proof of Lemma~\ref{teo:gulp}
(see~\cite{gulpinarI} for more details).
Finally, in Step $3$, we replaced the degree-greedy algorithm~\cite{paschos92} used in~\cite{gulpinarI} and~\cite{gutin09}
by an efficient stable set GRASP~\cite{feo94}.
We set the GRASP to halt after $100$ iterations have been performed since the last time the best solution was updated
or when a time limit of $300$ seconds is reached.

\subsection{A GRASP metaheuristic}

%{\color{red} YURI: //
%   motivacao para implementar um grasp //
%   descricao do grasp }

%It is well-known that enumerative procedures (e.g. a branch-and-cut) can largely benefit from
%high quality primal bounds since they allow for early pruning.
%
GRASP heuristics have been successfully applied to a large number of combinatorial optimization problems~\cite{marti13};
see~\cite{Festa} for a detailed annotated bibliography.
In  order  to  generate   better heuristic solutions  for  the
MBSP,   a   GRASP   heuristic is developed in this section.
The GRASP heuristic is an iterative  procedure that has two phases associated with each
iteration: a {\em  construction phase} and a  {\em  local search  phase}.
The construction phase  finds an initial solution that later might be
improved  by the  local  search phase.
Both phases are repeated until a termination criterion is satisfied.
In the remainder of this section, we describe these two phases.

The input  for  the heuristic is the signed graph $G=(V,E,s)$.
We assume that a feasible solution for the MBSP is defined as a pair of disjoint
sets $(V_1,V_2)$ such that $V_1,V_2 \subseteq V$, $E[V_1] \cup E[V_2] \subseteq E^+$
and $(E[V_1 \cup V_2] \backslash (E[V_1] \cup E[V_2])) \subseteq E^-$.

\paragraph{\bf Construction phase}
The overall method attempts to find a maximal feasible solution $(V_1,V_2)$.
The {\em construction phase} begins with $V_1=V_2=\emptyset$ and enlarges these
sets in a greedy way by adding one new vertex to the solution (to $V_1$ or to $V_2$) at a time.
Let $(V_1,V_2)$ be a feasible solution. We define
$Cand(V_1) = \{ i \in V  \backslash  (V_1 \cup V_2) \mid (V_1 \cup \{i\},V_2)\mbox{ is a feasible solution for the MBSP} \},$
as the set of  vertices that are candidate to enter the set $V_1$.
Similarly, we define
$Cand(V_2) = \{ i \in V  \backslash  (V_1 \cup V_2) \mid (V_1,V_2 \cup \{ i \}) \mbox{ is a feasible solution for the MBSP} \}.$
At each  iteration, a vertex $i  \in Cand(V_w)$ (for $w=1,2$) is randomly  selected and a
new set $V_w'$ is reached by inserting vertex $i$ into the set $V_w$.
%
The procedure is repeated until $Cand(V_1)=Cand(V_2)=\emptyset$.


\paragraph{\bf Local search phase}
Obviously, there is no guarantee that the construction phase returns a global optimal solution.
Therefore,  the solution $(V_1,V_2)$  may  be  improved by  a {\em  local search} procedure.
The neighborhood of the current solution $(V_1,V_2)$  is defined as the family of
all  pairs  $(V_1',V_2')$  obtained  by  applying one  of  the  following operations for $w\in \{1,2\}$:

\begin{itemize}
\item[] {\bf (i)}  removing a vertex $i$ from  $V_w$ and inserting a  vertex
$j \in (Cand(V_w \backslash \{ i \}) \cup Cand(V_{w\mod2}))$ into the corresponding subset (i.e. $V_w$ if
$j \in Cand(V_w \backslash \{ i \})$ and $V_{w\mod2}$ otherwise).
\vspace{- .2cm}
\item[] {\bf (ii)} removing two vertices $i_1$ and $i_2$ from  $V_w$ and inserting vertices $j_1$ and $j_2$ belonging to
$(Cand(V_w \backslash \{ i_1 , i_2 \}) \cup Cand(V_{w\mod2}))$ into the corresponding subsets.
\end{itemize}

%The neighborhoods {\bf (i)} and {\bf (ii)} are also applied dropping, respectively, one and two vertices from $V_2$.
The procedure  starts with the  solution provided by  the construction
phase and  iteratively replaces the  current solution by the  one with
maximum cardinality within its neighborhood, halting  when no better
solution is found in that way.
Similar to the stable set GRASP of Feo {\it et al.}~\cite{feo94}, the method stops after $100$ iterations have
been performed or when a time limit of $300$ seconds is reached.


